Doubly Optimal No-Regret Learning in Monotone Games

We consider online learning in multi-player smooth monotone games. Existing algorithms have limitations such as (1) being only applicable to strongly monotone games; (2) lacking the no-regret guarantee; (3) having only asymptotic or slow $O(\frac{1}{\sqrt{T}})$ last-iterate convergence rate to a Nash equilibrium. While the $O(\frac{1}{\sqrt{T}})$ rate is tight for a large class of algorithms including the well-studied extragradient algorithm and optimistic gradient algorithm, it is not optimal for all gradient-based algorithms. We propose the accelerated optimistic gradient (AOG) algorithm, the first doubly optimal no-regret learning algorithm for smooth monotone games. Namely, our algorithm achieves both (i) the optimal $O(\sqrt{T})$ regret in the adversarial setting under smooth and convex loss functions and (ii) the optimal $O(\frac{1}{T})$ last-iterate convergence rate to a Nash equilibrium in multi-player smooth monotone games. As a byproduct of the accelerated last-iterate convergence rate, we further show that each player suffers only an $O(\log T)$ individual worst-case dynamic regret, providing an exponential improvement over the previous state-of-the-art $O(\sqrt{T})$ bound.

==> macro.tex <==
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\usepackage[table,xcdraw]{xcolor}

\newcommand{\reg}{\text{Reg}}
\newcommand{\sreg}{\text{SReg}}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}
\DeclareRobustCommand\iff{\;\Longleftrightarrow\;}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\Graph}{Gra}


\newcommand{\notshow}[1]{{}}
\newcommand{\AutoAdjust}[3]{{ \mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }}
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}
\newcommand{\InAngles}[1]{\AutoAdjust{\langle}{#1}{\rangle}}
\newcommand{\InNorms}[1]{\AutoAdjust{\|}{#1}{\|}}
\renewcommand{\part}[2]{\frac{\partial #1}{\partial #2}}

\renewcommand{\P}{\mathcal{P}}
\newcommand{\R}{\mathbbm{R}} 
\newcommand{\N}{\mathcal{N}}

\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\C}{\mathcal{C}}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\prox}{\mathbf{Prox}}
\newcommand{\PP}{\mathbf{PP}}
\newcommand{\dg}{\mathsf{dg}}
\newcommand{\ham}{\mathsf{H}}
\newcommand{\Dom}[1]{\mathbf{dom}~#1}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}
\newcommand{\hZ}{\widehat{\Z}}
\newcommand{\hF}{\widehat{F}}
\newcommand{\hH}{\widehat{H}}
\newcommand{\oalpha}{\overline{\alpha}}
\newcommand{\obeta}{\overline{\beta}}
\newcommand{\ba}{\overline{a}}
\newcommand{\bb}{\overline{b}}
\newcommand{\bz}{\overline{z}}
\newcommand{\be}{\overline{e}}
\newcommand{\bZ}{\overline{Z}}
\newcommand{\bF}{\overline{F}}
\newcommand{\bx}{\overline{x}}
\newcommand{\bw}{\overline{w}}
\newcommand{\boldx}{\boldsymbol{x}}
\newcommand{\boldy}{\boldsymbol{y}}
\newcommand{\boldzero}{\boldsymbol{0}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hS}{\widehat{S}}
\newcommand{\supp}{\mathbf{Supp}}
\newcommand{\newpoint}[1]{#1_{\mathsf{new}}}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\indSet}{\mathbbm{I}}
\newcommand{\real}{\mathbbm{R}}
\newcommand{\ha}{\hat{a}}
\newcommand{\hb}{\hat{b}}
\newcommand{\tar}{\textsc{Target}}
\newcommand{\gap}{\textsc{Gap}}
\newcommand{\tgap}{\textsc{TGap}}
\newcommand{\sos}{\textsc{SOS}}
\newcommand{\LHSI}{\text{LHS of Inequality}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\ball}[2]{\mathcal{B}({#1},{#2})}
%\newcommand{\bw}{\boldsymbol{w}}

\newcommand{\LHSE}{\text{LHS of Equation}}

\newcommand{\RHSE}{\text{RHS of Equation}}

\newcommand{\Term}{\text{Expression}}
\newcommand{\term}{\textbf{term}}

\newenvironment{prevproof}[2]{\noindent {\bf {Proof of {#1}~\ref{#2}:}}}{$\hfill \square$}

\newenvironment{nalign}{    
\begin{equation}
    \begin{aligned}
}{
    \end{aligned}
    \end{equation}
    \ignorespacesafterend
}

%% MISC

% \newcommand{\note}[1]{{\color{green}{#1}}}
% \newcommand{\yangnote}[1]{{\color{cyan}{#1}}}
% \newcommand{\argyrisnote}[1]{{\color{magenta}{#1}}}
% \newcommand{\weiqiangnote}[1]{{\color{red}{#1}}}

% \newcommand{\yang}[1]{\todo[inline,size=footnotesize,color=blue!50]{\textbf{Yang:} {#1}}}

% \newcommand{\argyris}[1]{\todo[inline,size=footnotesize,color=red!20]{\textbf{Argyris:} {#1}}}

% \newcommand{\weiqiang}[1]{\todo[inline,size=footnotesize,color=green!20]{\textbf{Weiqiang:} {#1}}}

==> related_works.tex <==
\section{Potential Societal Impact}\label{sec:sociatal impact}
This work provides theoretical results for the convergence rate of  online learning algorithms in multi-player games. 
%Due to the theoretical nature, we expect that direct societal impact of this work will be limited. 
Online learning in multi-player games is a mathematical model that captures the strategic interaction between agents in multi-agent systems. From this perspective, our convergence results provide new  understandings of the evolution of the overall behavior of agents in multi-agent systems. More specifically, our results imply that certain natural dynamics will lead the agents' joint action profile to a stable state, i.e., a Nash equilibrium, efficiently. As a direct application, a designer of a multi-agent system can prescribe the learning algorithms studied in this paper, i.e., accelerated optimistic gradient, to agents, so that the system stabilizes quickly. Moreover, practical applications of min-max optimization (a special case of the games studied in this paper) include Generative Adversarial Networks (GANs) and adversarial examples. Therefore, our results might also provide useful insights on the training of GANs and adversarial training. To our best knowledge, we do not envision any immediate negative societal impacts of our results, such as security, privacy, and fairness issues.

\section{Related Works}
\paragraph{Last-Iterate Convergence of No-regret learning in Games} 
%Learning in games is a fundamental topic in the intersection of game theory and machine learning. 
There is a vast literature on no-regret learning in games. For strongly monotone games, linear last-iterate convergence rate is known~\cite{tseng_linear_1995,liang_interaction_2019,mokhtari_convergence_2020,zhou_convergence_2020}. Even under bandit feedback or noisy gradient feedback, optimal sub-linear last-iterate convergence rate is achieved by no-regret learning algorithms for strongly monotone games~\cite{lin_doubly_2022, jordan2022adaptive}.


Obtaining last-iterate convergence rate to Nash equilibria beyond strongly monotone games received extensive attention recently. \cite{daskalakis_limit_2018} proved asymptotic convergence of the optimistic gradient \eqref{OG} algorithm in zero-sum games. Asymptotic convergence was also achieved in variationally stable games~\cite{zhou_mirror_2017,zhou_countering_2017, mertikopoulos_learning_2018,hsieh2021adaptive} even with noisy feedback~\cite{hsieh2022no}. Finite time $\mathcal{O}(\frac{1}{\sqrt{T}})$ convergence was shown for unconstrained cocoercive games~\cite{lin_finite-time_2020} and unconstrained monotone games~\cite{golowich_tight_2020}. For bilinear games over polytopes, \cite{wei_linear_2021} show linear convergence rate of \ref{OG} but this rate depends on a problem constant $c$ which can be arbitrarily large. Recently, \cite{cai_finite_22} proved a tight $\mathcal{O}(\frac{1}{\sqrt{T}})$ last-iterate convergence rate of \ref{OG} and the extragradient (EG) algortihm for constrained monotone games, matching the lower bound of p-SCIL algorithms by~\cite{golowich_tight_2020}. We remark that for general gradient-based algorithms, the lower bound is $\Omega(\frac{1}{T})$~\cite{ouyang2021lower,yoon_accelerated_2021}. 


\paragraph{Regret Minimization in Games}
There is a large body of works on minimizing  individual regret in games, from early results in two-player zero-sum games~\cite{daskalakis2011near,kangarshahi2018let} to more recent works on general-sum games~\cite{syrgkanis_fast_2015,chen_hedging_2020, daskalakis_near-optimal_2021,anagnostides_near-optimal_2021, anagnostides_uncoupled_2022}. Among them, \cite{daskalakis_near-optimal_2021,anagnostides_near-optimal_2021, anagnostides_uncoupled_2022} achieves $\mathcal{O}(\log T)$ regret for general-sum games and \cite{hsieh2021adaptive} achieves $\mathcal{O}(1)$ regret for variationally stable games. Little is known, however, for the stronger notion of dynamic regret except for $\mathcal{O}(\sqrt{T})$ bound of \ref{OG} in monotone games~\cite{cai_finite_22}. 
